Hyperspectral Lightcurve Inversion for Attitude Determination

Spectral lightcurves consisting of time series single-pixel spectral measurements of spacecraft are used to infer the spacecraft's attitude and rotation. Two methods are used. One based on numerical optimisation of a regularised least squares cost function, and another based on machine learning with a neural network model. The aim is to work with minimal information, thus no prior is available on the attitude nor on the inertia tensor. The theoretical and practical aspects of this task are investigated, and the methodology is tested on synthetic data. Results are shown based on synthetic data.

==> 20_single_spectrum.tex <==
\section{Attitude from a single spectrum observation}
\label{sec:single_spectrum}

Conceptually, the observation at an instant in time is the intensity of light received as a function of wavelength $S(\lambda)$.
This function depends on the direction of incident light $\hat{\bf s}_B$ and the view direction $\hat{\bf s}_B$, where the subscript $B$ indicates these vectors are written in the body frame.
We can therefore write $S(\lambda) = S(\lambda; \hat{\bf v}_B, \hat{\bf s}_B)$, where $\hat{\bf v}_B$ and $\hat{\bf s}_B$ are unknown, but the angle between them, the phase angle $\alpha$, is known.

In this work we assume accurate knowledge of the view and illumination directions in the inertial frame, $\hat{\bf v}_I$ and $\hat{\bf s}_I$ (from which we also know $\alpha$), since these can be obtained from basic knowledge of astro-dynamics and measurement geometry.
If $\alpha \notin \{0, \pi\}$, the attitude of the body is determined from $\hat{\bf v}_B$ and $\hat{\bf s}_B$, by finding the rotation $R$ that makes $\hat{\bf v}_I = R\hat{\bf v}_B$ and $\hat{\bf b}_I = R\hat{\bf b}_B$.
Therefore, we wish to find the vectors $\hat{\bf v}_B$ and $\hat{\bf s}_B$ that make the observed spectra $\hat{S}(\lambda)$ match the theoretically obtained $S(\lambda; \hat{\bf v}_B, \hat{\bf s}_B)$, with the constraint on the known phase angle $\alpha$. This is formulated as a least squares (LS) problem,
\begin{equation} \label{eq:spec_min}
\begin{split}
    \min_{\hat{\bf v}_B, \hat{\bf s}_B}&
    \int \left\lvert \hat{S}(\lambda) -  S(\lambda; \hat{\bf v}_B, \hat{\bf s}_B) \right\rvert^2 \ud\lambda \\
    {\rm s.t.}~ & \lVert \hat{\bf v}_B \rVert = 1 \\
    & \lVert \hat{\bf s}_B \rVert = 1 \\
    & \hat{\bf v}_B \cdot \hat{\bf s}_B = \cos{\alpha}
\end{split}
\end{equation}

% \begin{table}[b]
%     \centering\small
%     \caption{Abundances of each material for the first test cube. Material spectra collected in lab experiments. Source: \cite{walker_2022_hyperspectral}.}
%     \label{tab:complex_cube}
%     \begin{tabular}{cccc}
%     \toprule
%     \thead{Cube face\\(body axis)}	& \thead{Aluminium foil\\fraction} & \thead{Gold foil\\fraction} & \thead{Solar panel\\fraction} \\
%     \midrule
%         $+x$ & 0.5 & 0 & 0.5 \\
%         $+y$ & 0 & 0 & 1 \\ 
%         $+z$ & 0.5 & 0.5 & 0 \\ 
%         $-x$ & 0.75 & 0 & 0.25 \\ 
%         $-y$ & 0 & 0.135 & 0.865 \\ 
%         $-z$ & 0 & 0.5 & 0.5\\ 
%         \bottomrule
%     \end{tabular}
% \end{table}

As an experiment, this strategy is applied to simulated observations of the cubic object used in \cite{walker_2022_hyperspectral}, with a purely Lambertian model for $S$, and with each surface covered in different mixtures of three materials.
A convex object can be described for these purposes with a facet model, consisting of a set of $N$ faces, where the $i$-th face's normal is ${\bf n}_i$ and its average colour is ${\bf c}_i(\lambda)$. 
Average colour here means the average reflectance spectrum of the face in question multiplied by its area. The Lambertian model can thus be written as
\begin{equation} \label{eq:Lambert}
    S(\lambda; \hat{\bf v}_B, \hat{\bf s}_B)
    =
    \sum_{i=1}^N
    \max(0, \hat{\bf v}_B \cdot {\bf n}_i)
    \max(0, \hat{\bf s}_B \cdot {\bf n}_i)
    {\bf c}_i(\lambda)
    ~.
\end{equation}

A consequence of the Lambertian and other models \cite{muinonen_asteroid_2020} is that the view and illumination angles can be swapped and this will result in the same observation, i.e. $S(\lambda; \hat{\bf v}_B, \hat{\bf s}_B) = S(\lambda; \hat{\bf s}_B, \hat{\bf v}_B)$, which results in an ambiguity in the attitude determination process. 
To this are added other ambiguities that may result from the object, even if it is asymmetric.
The bisector $\hat{\bf h}$ is the vector in between $\hat{\bf v}$ and $\hat{\bf s}$, also known as the phase vector, and defined as
\begin{equation}
    \bf \hat{h} = \frac{\hat{s} + \hat{v}}{\lVert \hat{s} + \hat{v} \rVert}
\end{equation}
Using this vector tends to be better for describing the appearance of the object to multi-spectral imaging, as suggested in \cite{nussbaum_spectral_2022}, in part due to the previously mentioned symmetry.
A uniform sample of attitudes is obtained using the same energy based method used in \cite{ricciardi_improved_2019}.
The plots in Fig. \ref{fig:local_optima} show the local optima for the view and illumination directions for the same cube with its +x face aligned with the bisector.
They are very similar due to the symmetry mentioned previously.
The circles each define a set where the spectrum generated is exactly the same, and they include the set of global optima. These circles have as centres the phase vector $\bf \hat{h}$, which is approximately the same for each of those circles.


\begin{figure}
     \centering
     \begin{subfigure}[b]{0.47\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/illum_103.eps}
         \caption{$\hat{\bf v}_B$}
         \label{fig:local_optima:v}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.47\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/view_103.eps}
         \caption{$\hat{\bf s}_B$}
         \label{fig:local_optima:s}
     \end{subfigure}
     \caption{Local optima for $\hat{\bf v}_B$ and $\hat{\bf s}_B$ }
     \label{fig:local_optima}
\end{figure}


Let us now consider a parameterization using the azimuth $\theta_h$ and elevation $\phi_h$ of the phase vector, such that
\begin{equation}
    \hat{\bf h}_B = R_z(\theta_B) R_y(-\phi_B) \hat{\bf x}
\end{equation}
where $R_a(\theta)$ represents a rotation around vector $\hat{\bf a}$ of angle $\theta$.
In addition, the roll angle $\psi_h$ is used, which, along with the phase angle $\alpha$, define the view and illumination vectors as
\begin{align}
    \hat{\bf v}_B &= R_z(\theta_h) R_y(-\phi_h) R_x(\psi_h) R_z(\alpha/2) \hat{\bf x} \\
    \hat{\bf s}_B &= R_z(\theta_h) R_y(-\phi_h) R_x(\psi_h) R_z(-\alpha/2)\hat{\bf x}
\end{align}
These are Euler angles used to visualise the behaviour of this cost function. 
The cost function $J$ is still to be optimised as a function of $\hat{\bf s}_B$ and $\hat{\bf v}_B$ as in Eq. (\ref{eq:spec_min}).

A contour plot of $\min_{\psi_h} J(\theta_h, \phi_h, \psi_h)$ is in Fig. \ref{fig:map_002}.
It shows a unique optimum $\theta_h^*, \phi_h^*$ for this case.
However, it is seen that $J(\psi_h) = J(\theta_h^*, \phi_h^*, \psi_h)$ is a constant function, showing that there is not a single global optimum over $\hat{\bs v}_B$ and $\hat{\bs s}_B$, but in this case a whole continuous set of global optima.

\begin{figure}
    \centering%[trim={left bottom right top},clip]
    \includegraphics[trim={0 0 0 0.38cm},clip]{Figures/map_of_cost_function_value_for_bisector_-_i=103.eps}
    \caption{Contour plot of $\min_{\psi_h} J(\theta_h, \phi_h, \psi_h)$ when the observed spectrum corresponds to $\theta_h=\phi_h=\psi_h=0$.}
    \label{fig:map_002}
\end{figure}

In another example where there the x axis of the object is at an angle of 32 degrees to the phase vector, this type of ambiguity also occurs, albeit somewhat differently.
Figure \ref{fig:map_prev} shows the same contour plot, this time with a circular level set containing the real solution, and a sample of local optima that are all also global optima.
For completion, a plot of $J(\psi_h) = J(\theta_h^*, \phi_h^*, \psi_h)$ is shown in Fig \ref{fig:rot_h}, also showing a function that is almost piecewise constant.


\begin{figure}
    \centering
    %[trim={left bottom right top},clip]
    \includegraphics[trim={0 0 0 0.38cm},clip]{Figures/map_of_cost_function_value_for_bisector_-_i=001.eps}
    \caption{Contour plot of $\min_{\psi_h} J(\theta_h, \phi_h, \psi_h)$ for the scenario where $\hat{\bf h} \cdot \hat{\bf x} = \cos(32 ^\circ)$.}
    \label{fig:map_prev}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{Figures/Rotation_about_bisector_-_i=001.eps}
    \caption{Plot of $J(\psi_h) = J(\theta_h^*, \phi_h^*, \psi_h)$ for the scenario where $\hat{\bf h} \cdot \hat{\bf x} = \cos(32 ^\circ)$.}
    \label{fig:rot_h}
\end{figure}
